Enhancing the Energy Efficiency of Radio Base Stations

This thesis is concerned with the energy efficiency of cellular networks. It studies the dominant power consumer in future cellular networks, the Long Term Evolution radio base stations (BS), and proposes mechanisms that enhance the BS energy efficiency by reducing its power consumption under target rate constraints. These mechanisms trade spare capacity for power saving.

==> thesis/README <==
Template for a LaTeX PhD UoE Thesis.
====================================

Author: Magnus Hagdorn

This template setup allows you to produce:
* a thesis that adheres to the UoE regulations
  (at least my interpretations of them and no-one complained when
  I submitted mine)
* a nicely formatted pdf/ps version of the same thesis
  with single line spacing, etc
* individual documents for each chapter

Indivdual chapters reside in their own directories. (Re)-Define the macro \dir
to the relative path where files for the current chapter can be found. You can
then use \dir to include files or graphics, e.g.

\newcommand{\dir}{theory}
\input{\dir/theory.tex}
\epsfig{file=\dir/images/test.eps,width=0.5\textwidth}

Using this macro allows you to distribute files over a number of directories.

The common directory
--------------------
This directory contains files used by all the documents:
* the packages.tex files contains a lits of packages used
* the definitions.tex file contains settings and macros

The preface directory
---------------------
contains files for the preface.

The template directory
----------------------
This directory should be copied for each chapter. Rename the sub directory 
accordingly. All files should be kept in this sub directory. If you want to
produce a document for the individual chapter, run latex on the chapter.tex
file.

The thesis directory
--------------------
This directory pulls files from the preface and the chapter directories together
to produce the complete thesis. There are 3 different top level files:
* latex ed_thesis.tex
  to produce official 1.5 (?) spaced thesis which adheres to the regulations
* latex nicepdf_thesis.tex
  to produce a dvi file to be processed using dvipdft. The resulting pdf will
  have colour hyperlinks.
* latex niceps_thesis.tex
  to produce a single spaced thesis without the hyperlinks for printing

All three top level files include the thesis.tex file. This file includes the
actual preface and chapter files. 

You can use the \ifthenelse macro to do specific things for either the standard
or nice thesis version, e.g.
\ifthenelse{\boolean{edthesis}}
 {
   Do something specific for the offical version 
}
{
   Do something else for the nice version
}



If you have any questions or problems contact IThelp@geos.ed.ac.uk.

